On-Stack Replacement \`a la Carte

On-stack replacement (OSR) dynamically transfers execution between different code versions. This mechanism is used in mainstream runtime systems to support adaptive and speculative optimizations by running code tailored to provide the best expected performance for the actual workload. Current approaches either restrict the program points where OSR can be fired or require complex optimization-specific operations to realign the program's state during a transition. The engineering effort to implement OSR and the lack of abstractions make it rarely accessible to the research community, leaving fundamental question regarding its flexibility largely unexplored. In this article we make a first step towards a provably sound abstract framework for OSR. We show that compiler optimizations can be made OSR-aware in isolation, and then safely composed. We identify a class of transformations, which we call live-variable equivalent (LVE), that captures a natural property of fundamental compiler optimizations, and devise an algorithm to automatically generate the OSR machinery required for an LVE transition at arbitrary program locations. We present an implementation of our ideas in LLVM and evaluate it against prominent benchmarks, showing that bidirectional OSR transitions are possible almost everywhere in the code in the presence of common, unhindered global optimizations. We then discuss the end-to-end utility of our techniques in source-level debugging of optimized code, showing how our algorithms can provide novel building blocks for debuggers for both executables and managed runtimes.

==> osr-correctness.tex <==
% !TEX root = ms.tex

\subsection{Algorithm Correctness}
\label{ss:osr-mapping-correctness}

\oldrevision{
We now prove the correctness of ${\tt OSR\_trans}$, showing that it yields strict OSR mappings if the applied rewrite rules satisfy the property that variables that are live at corresponding points in the original and rewritten program contain the same values. To characterize this property, we need to introduce some formal machinery based on bisimilarity of programs.


\begin{definition}[Program Bisimulation]
\label{de:bisimulation}
A relation $R\subseteq State\times State$ is a bisimulation relation between two programs $\pi$ and $\pi'$ if for any input store $\sigma\in \Sigma$ it holds:
\begin{align*}
s\in\tau_{\pi\sigma} ~ & \wedge ~~ s'\in \tau_{\pi'\sigma} ~~ \wedge ~~ s~R~s' \Longrightarrow \\
1) & ~~ s\Rightarrow_{\pi} s_1 ~~~ \Longrightarrow ~~~ s'\Rightarrow_{\pi'} s'_1 ~~ \wedge  ~~ s_1~R~s'_1 \\
2) & ~~ s'\Rightarrow_{\pi'} s'_1 ~~~ \Longrightarrow ~~~ s\Rightarrow_{\pi} s_1 ~~ \wedge  ~~ s_1~R~s'_1
\end{align*}
\end{definition}


\noindent Notice that our notion of bisimulation between programs $\pi$ and $\pi'$ requires that $R$ be a bisimulation between transition systems $(\tau_{\pi\sigma}, \Rightarrow_{\pi})$ and $(\tau_{\pi'\sigma}, \Rightarrow_{\pi'})$ for any store $\sigma\in \Sigma$. %This implies that for any $\sigma$, $\tau_{\pi\sigma}$ is finite if and ony if $\tau_{\pi'\sigma}$ is finite; also, if they are finite, then they have the same length.

\begin{restatable}{lem}{bisimprop}
\label{le:bisim-prop}
Let $R$ be a reflexive bisimulation relation between programs $\pi$ and $\pi'$. Then for any $\sigma\in \Sigma$ it holds:
\begin{equation}
\label{eq:bisim-prop-1}
|\tau_{\pi\sigma}|=|\tau_{\pi'\sigma}|
\end{equation}
\begin{equation}
\label{eq:bisim-prop-2}
\forall i\in dom(\tau_{\pi\sigma}), ~~ \tau_{\pi\sigma}[i]~R~\tau_{\pi'\sigma}[i]
\end{equation}
\end{restatable}
% proof moved to appendix

\begin{definition}[Partial State Equivalence]
\label{de:state-equiv-relation}
For any function $A:\mathbb{N}\rightarrow 2^{Var}$, the {\em partial state equivalence} relation $R_A\subseteq State\times State$ is defined as:
\begin{equation*}
%\begin{split}
%R_A\triangleq\{ & (s, s')\in State\times State ~ | ~  \\
%& s=(\sigma,l) ~ \wedge ~ s'=(\sigma',l) ~ \wedge ~ \sigma\vert_{A(l)} = \sigma'\vert_{A(l)} \}.
%\end{split}
R_A\triangleq\{ (s, s')\in State\times State ~ | ~  s=(\sigma,l) ~ \wedge ~ s'=(\sigma',l) ~ \wedge ~ \sigma\vert_{A(l)} = \sigma'\vert_{A(l)} \}.
\end{equation*}
\end{definition}

\noindent Relation $R_A$ is clearly reflexive, symmetric, and transitive.

\begin{definition}[Live-Variable Bisimilar Programs]
\label{de:lvb-programs}
$\pi$ and $\pi'$ are {\em live-variable bisimilar} (LVB) if $R_{A}$ is a bisimulation relation between them, where $A=l\mapsto\live(\pi,l)\cap \live(\pi',l)$ is the function that yields for each program point $l$ the set of variables that are live at $l$ in both $\pi$ and $\pi'$.
\end{definition}


\noindent One consequence of \mydefinition\ref{de:state-equiv-relation}, which simplifies our formal discussion, is the following:

\begin{restatable}{lem}{lvbsameloc}
\label{le:lvb-same-loc}
If $\pi$ and $\pi'$ are live-variable bisimilar, then for any $\sigma$, corresponding states in program traces $\tau_{\pi\sigma}$ and $\tau_{\pi'\sigma}$ are located at the same program points: $\forall i:$ $\tau_{\pi\sigma}[i]=(\sigma_i, l_i)$ $\wedge$ $\tau_{\pi'\sigma}[i]=(\sigma'_i, l'_i)$ $\Longrightarrow$ $l_i=l'_i$.
\end{restatable}
% proof moved to appendix

\begin{restatable}{cor}{samesize}
\label{co:same-size}
If $\pi$ and $\pi'$ are live-variable bisimilar, then they have the same size: $\pi=\langle I_1,\ldots,I_n\rangle$ $\wedge$ $\pi'=\langle I'_1,\ldots,I'_{n'}\rangle$ $\Longrightarrow$ $n=n'$.
\end{restatable}
}
% moved to appendix

\oldrevision{
\noindent We can now prove that \buildcomp\ generates correct OSR compensation code under the live-variable bisimilarity assumption.

\begin{restatable}[Correctness of Algorithm \buildcomp]{lem}{buildcompcorr}
\label{le:build-comp-corr}
Let $\pi$ and $\pi'$ be live-variable bisimilar programs. For each initial store $\sigma\in \Sigma$ it holds:
\begin{equation*}
\forall i\in dom(\tau_{\pi\sigma}): \chi\neq undef \implies
\mysem{\chi}(\sigma_i\vert_{\live(\pi,l_i)}) = \sigma'_i\vert_{\live(\pi',l_i)}
\end{equation*}
where $(\sigma_i,l_i)=\tau_{\pi\sigma}[i]$, $(\sigma'_i,l_i)=\tau_{\pi'\sigma}[i]$, and $\chi={\tt build\_comp}(\pi,l_i,\pi',l_i)$.
\end{restatable}
% proof moved to appendix


\begin{definition}[Live-Variable Equivalent Transformation]
\label{de:lve-trans}
A program transformation $T$ is {\em live-variable equivalent} (LVE) if for any program $\pi$, $\pi$ and $\mysem{T}(\pi)$ are live-variable bisimilar.
\end{definition}
}

\oldrevision{
\noindent We can finally establish the correctness of ${\tt OSR\_trans}$, which follows directly by \mylemmas\ref{le:lvb-same-loc} and~\ref{le:build-comp-corr} and \mycorollary\ref{co:same-size}:

}

